Perceive, Attend, and Drive: Learning Spatial Attention for Safe Self-Driving

In this paper, we propose an end-to-end self-driving network featuring a sparse attention module that learns to automatically attend to important regions of the input. The attention module specifically targets motion planning, whereas prior literature only applied attention in perception tasks. Learning an attention mask directly targeted for motion planning significantly improves the planner safety by performing more focused computation. Furthermore, visualizing the attention improves interpretability of end-to-end self-driving.

==> sections/tab_main_nusc.tex <==
% !TEX root = ../main.tex
\setlength{\tabcolsep}{6pt}
\captionsetup[table]{skip=10pt}
\begin{table}[t]
\centering
\begin{small}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
\multirow{2}{*}{\bf{Model}} & \bf{Backbone} & \multirow{2}{*}{\bf{Sparsity}} & \bf{Planning L2} & \bf{Lane Violation} & \multicolumn{3}{c|}{\bf{mAP @ IOU}} \\
& \bf{FLOPS} & & \bf{over 3s (m)} & \bf{over 3s (\%)} & \bf{0.3} & \bf{0.5} & \bf{0.7} \\\hline

Original NMP            & 39.18B      &  0.0\%      & 2.310      & 1.918      & \bf{81.7} & \bf{77.6} & \bf{60.6} \\
Dense NMP               & 22.73B      &  0.0\%      & 2.271      & 2.198      & 78.2      & 73.7      & 53.7 \\
\hline
NMP+Proximity Mask      & 5.41B       & \bf{94.0}\%      & 2.103      & 2.073      & 61.4      & 55.2      & 40 \\
NMP+Learned Attn (Ours) & \bf{5.34B}  & \bf{94.0\%} & \bf{2.052} & \bf{1.588} & 76.9      & 71.4      & 54.7 \\
\end{tabular}}
\end{small}
\caption{Motion planning performance and computational efficiency of our learned sparse attention model vs. other baselines}
\label{tab:mainnusc}
\end{table}

